Context-Aware Entity Grounding with Open-Vocabulary 3D Scene Graphs

We present an Open-Vocabulary 3D Scene Graph (OVSG), a formal framework for grounding a variety of entities, such as object instances, agents, and regions, with free-form text-based queries. Unlike conventional semantic-based object localization approaches, our system facilitates context-aware entity localization, allowing for queries such as ``pick up a cup on a kitchen table" or ``navigate to a sofa on which someone is sitting". In contrast to existing research on 3D scene graphs, OVSG supports free-form text input and open-vocabulary querying. Through a series of comparative experiments using the ScanNet dataset and a self-collected dataset, we demonstrate that our proposed approach significantly surpasses the performance of previous semantic-based localization techniques. Moreover, we highlight the practical application of OVSG in real-world robot navigation and manipulation experiments.

==> Sections/4_experiment-before-refactoring.tex <==
We performed experiments on our OVSG (Open Vocabulary Semantic Grounding) framework to address the following research questions: 1) How do our context-aware grounding methods outperform the SOTA semantic grounding method OVIR-3D? 2) How is OVSG performing in terms of open-vocabulary queries? 3) How do our graph similarity-based methodologies perform differently? 4) How can our system be integrated into the real robot environment?

\subsection{Dataset Preparation and Metrics}
\textbf{ScanNet} We are using the validation chunk from the state-of-the-art ScanNet dataset for evaluation, consisting of 312 scenes. 
ScanNet dataset only has objects, hence we simulate agents and induce their abstract relationships to objects, capture spatial relationships between objects, and utilize the OVIR-3D method to extract object features before incorporating the dataset into the evaluation pipeline. Due to resource constraints, we could not manually label ScanNet's 312 scenes and therefore synthetically generated 43000 queries for evaluation (refer to Appendix~\ref{appendix:a} for details). 

\textbf{DOVE-G} To accommodate the richness of open-vocabulary queries, we introduced a custom dataset—DOVE-G (Dataset for Open-Vocabulary Entity Grounding). This is to facilitate users to query for objects within a scene using natural language. For each scene within DOVE-G, we manually labeled the ground truth and created 50 natural language queries ($L_{q}$). To augment this query set, we harnessed LLMs to generate four additional sets of natural language queries. This approach yielded a total of 250 queries for each scene, and cumulatively, we have 4000 queries to evaluate OVSG's performance. With this setup, we set out to assess how our OVSG framework performs with open-vocabulary queries, one of our key research questions, providing a critical testbed for its effectiveness in handling diverse natural language expressions. 

\begin{table}[htbp]
\centering
% \resizebox{\columnwidth}{!}{%
\scalebox{0.5}{
\begin{tabular}{>{\centering\arraybackslash}m{2.5cm}cccccccc}
\toprule
\multirow{2}{*}{Metric} & \multicolumn{4}{c}{Top1 Scores} & \multicolumn{4}{c}{Top3 Scores} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\  
\midrule
Match Rate & 13.80 & 20.73 & 26.35 & \cellcolor{PaleBlue}\textbf{31.19} & 34.72 & 29.49 & 37.18 & \cellcolor{PaleBlue}\textbf{38.47} \\ 
IoU & 0.14 & 0.21 & 0.25 & \cellcolor{PaleBlue}\textbf{0.29} & 0.35 & 0.29 & 0.36 & \cellcolor{PaleBlue}\textbf{0.38} \\ 
\bottomrule
\end{tabular}
}
\caption{Overall Performance of the OVSG framework on the ScanNet dataset}
\label{tab:table4}
\end{table}

\begin{table}[htbp]
\centering
% \resizebox{\columnwidth}{!}{%
\scalebox{0.5}{
\begin{tabular}{>{\centering\arraybackslash}m{2.5cm}cccccccc}
\toprule
\multirow{2}{*}{Metric} & \multicolumn{4}{c}{Top1 Scores} & \multicolumn{4}{c}{Top3 Scores} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\  
\midrule
Match Rate & 35.2 & 25.2 & 45.4 & \cellcolor{PaleBlue}\textbf{51.1} & 63.6 & 47.1 & 64.8 & \cellcolor{PaleBlue}\textbf{65.7} \\ 
IoU & 0.28 & 0.18 & 0.34 & \cellcolor{PaleBlue}\textbf{0.39} & 0.49 & 0.39 & 0.49 & \cellcolor{PaleBlue}\textbf{0.50} \\ 
\bottomrule
\end{tabular}
}
\caption{Overall Performance of the OVSG framework on DOVE-G}
\label{tab:table1}
\end{table}
\textbf{Evaluation Metrics} For each query, we calculated IoU scores between the bounding boxes of the correct match (ground truth) and the top candidates returned by the system. We also measured the match rate for each scene, which refers to the percentage of queries where the bounding box of the predicted candidate overlapped with the ground truth with an IoU score of 0.5 or more. This threshold can be adjusted to alter the strictness of the match criteria. We reported the top-1 and top-3 match rates and average IoU scores for each scene, reflecting the performance of our system in the top-k results returned for each query.

\subsection{Baselines}
We evaluate four different methods in our experiments. The SOTA open-vocabulary grounding method, OVIR-3D, is our baseline as it will not leverage any inter-notion relations, providing a comparative measure for the effectiveness of contextual information integration in the other methods. The rest of the methods perform Context-Aware Entity Grounding by employing sub-graph matching techniques (refer to Subsection~\ref{sec:sub-graph-matching}). We denote those three graph similarity method variants as OVSG-J, OVSG-S, and OVSG-L (for Jaccard coefficient, Szymkiewicz-Simpson index, and Likelihood, respectively). 

% \begin{table}[htbp]
% \centering
% \scalebox{0.55}{
% \begin{tabular}{>{\centering\arraybackslash}m{2.5cm}cccccccc}
% \toprule
% \multirow{2}{*}{Scene} & \multicolumn{4}{c}{Top1 Match Rate} & \multicolumn{4}{c}{Top3 Match Rate} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\ 
% \midrule
% Room \#1 & 44.4 & 36.8 & 61.2 & \cellcolor{PaleBlue}\textbf{79.6} & 88.4 & 72.8 & 98.4 & \cellcolor{PaleBlue}\textbf{99.6} \\
% Kitchenette & 31.0 & 24.0 & 36.0 & \cellcolor{PaleBlue}\textbf{49.0} & 65.0 & 51.0 & 71.0 & \cellcolor{PaleBlue}\textbf{71.0} \\ 
% Bathroom & 44.8 & 23.2 & 57.2 & \cellcolor{PaleBlue}\textbf{58.0} & 59.6 & 41.2 & 66.0 & \cellcolor{PaleBlue}\textbf{69.6} \\ 
% Kitchen & 44.8 & 36.0 & 51.2 & \cellcolor{PaleBlue}\textbf{55.6} & 53.6 & 50.8 & 55.2 & \cellcolor{PaleBlue}\textbf{56.8} \\ 
% Room \#2 & 18.0 & 26.0 & 40.0 & \cellcolor{PaleBlue}\textbf{41.6} & 62.0 & 48.0 & \textbf{65.2} & \cellcolor{PaleBlue}62.8 \\ 
% Computer Lab & 38.0 & 30.8 & 38.0 & \cellcolor{PaleBlue}\textbf{41.6} & \textbf{54} & 41.2 & 50.4 & \cellcolor{PaleBlue}49.2 \\
% Room \#3 & 32.8 & 16.8 & 40.4 & \cellcolor{PaleBlue}\textbf{40.4} & \textbf{47.2} & 34.4 & \textbf{47.2} & \cellcolor{PaleBlue}\textbf{47.2} \\ 
% Hallway & 28.0 & 8.4 & 28.4 & \cellcolor{PaleBlue}\textbf{33.2} & 40.0 & 34.4 & 40.0 & \cellcolor{PaleBlue}\textbf{40.0} \\ 
% \midrule
% Overall & 35.2 & 25.2 & 45.4 & \cellcolor{PaleBlue}\textbf{51.1} & 63.6 & 47.1 & 64.8 & \cellcolor{PaleBlue}\textbf{65.7} \\
% \toprule
% \multirow{2}{*} {} & \multicolumn{4}{c}{Top1 IoU} & \multicolumn{4}{c}{Top3 IoU} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\ 
% \midrule
% Room \#1 & 0.26 & 0.18 & 0.36 & \cellcolor{PaleBlue}\textbf{0.47} & 0.55 & 0.39 & 0.60 & \cellcolor{PaleBlue}\textbf{0.61} \\
% Kitchenette & 0.28 & 0.23 & 0.34 & \cellcolor{PaleBlue}\textbf{0.42} & 0.59 & 0.47 & 0.62 & \cellcolor{PaleBlue}\textbf{0.62} \\ 
% Bathroom & 0.30 & 0.13 & 0.36 & \cellcolor{PaleBlue}\textbf{0.36} & 0.41 & 0.30 & 0.44 & \cellcolor{PaleBlue}\textbf{0.46} \\ 
% Kitchen & 0.35 & 0.28 & 0.38 & \cellcolor{PaleBlue}\textbf{0.42} & 0.47 & 0.42 & 0.46 & \cellcolor{PaleBlue}\textbf{0.48} \\ 
% Room \#2 & 0.15 & 0.21 & 0.31 & \cellcolor{PaleBlue}\textbf{0.34} & 0.51 & 0.41 & \textbf{0.53} & \cellcolor{PaleBlue}0.52 \\ 
% Computer Lab & 0.32 & 0.22 & 0.33 & \cellcolor{PaleBlue}\textbf{0.39} & \textbf{0.49} & 0.39 & 0.45 & \cellcolor{PaleBlue}0.46 \\
% Room \#3 & 0.34 & 0.13 & 0.37 & \cellcolor{PaleBlue}\textbf{0.39} & 0.50 & 0.36 & 0.49 & \cellcolor{PaleBlue}\textbf{0.50} \\ 
% Hallway & 0.27 & 0.10 & 0.24 & \cellcolor{PaleBlue}\textbf{0.31} & 0.37 & 0.34 & 0.38 & \cellcolor{PaleBlue}\textbf{0.41} \\ 
% \midrule
% Overall & 0.28 & 0.18 & 0.34 & \cellcolor{PaleBlue} \textbf{0.39} & 0.49 & 0.39 & 0.49 & \cellcolor{PaleBlue}\textbf{0.50} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Performance of the OVSG framework on natural language scene queries in the Custom Dataset.}
% \label{tab:table1}
% \end{table}

\subsection{Performance}
\textbf{ScanNet}
Concerning the ScanNet dataset, we have averaged the scores for the 312 scenes and presented the results in Table~\ref{tab:table4}. From an overall perspective, leveraging contextual information for grounding entities proved useful as the graph similarity variants (OVSG-J, OVSG-S, OVSG-L) outperformed the SOTA semantic segmentation method (OVIR-3D). Especially, the OVIR-3D method performed poorly for scenes of type bookstore or library, or conference room where there are multiple instances of the same entity. Hence, a lack of context/specification for the target object being queried makes the object retrieval process less accurate. Moreover, the OVSG-L method significantly outperformed the other methods with an average Top1 Match Rate and IoU of 31.19\% and 0.29, respectively. The average Top3 Match Rate and IoU were also higher, at 38.47\% and 0.38, respectively. appendix:a1

\textbf{DOVE}
Table~\ref{tab:table1} summarizes the performance of all the methods across every scene in DOVE-G, averaged over all five sets of natural language queries. 
OVSG-L consistently outperforms other methods across all scenes.
For instance, in Room \#1, OVSG-L secures a Top1 match rate of 79.6\%, far exceeding the scores of OVIR-3D (44.4\%), OVSG-J (36.8\%), and OVSG-S (61.2\%). A similar trend is observed in the Kitchenette scene.
% , where OVSG-L delivers a match rate of 49.0\%, compared to 31.0\% (OVIR-3D), 24.0\% (OVSG-J), and 36.0\% (OVSG-S).
OVSG-J and OVSG-S also show competitive results in some scenes. 
% In Room \#2, for example, OVSG-S outperforms OVIR-3D in both Top1 (40.0\% vs 18.0\%) and Top3 (65.2\% vs 62.0\%) match rates. 
Despite these bright spots, both methods are generally overshadowed by OVSG-L's superior performance.
% The benefit of using contextual information becomes even more pronounced in certain environments, such as Room \#1 and the Kitchenette. 
% These improvements hold true across all metrics, although 
The OVIR-3D model does manage to stay competitive with the other three methods, particularly in the top-3 categories. Because scenes in DOVE-G do not contain a large number of identical instances as in a stack of several books in a library scene, the top-3 results returned by the system usually contain the ground truth match.
\begin{table}[htbp]
\centering
\begin{minipage}{.45\linewidth}
\centering
\scalebox{0.40}{
\begin{tabular}{>{\centering\arraybackslash}m{2.5cm}cccccccc}
\toprule
\multirow{2}{*}{Vocab Set} & \multicolumn{4}{c}{Top1 Match Rate} & \multicolumn{4}{c}{Top3 Match Rate} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\ 
\midrule
\#1 & 35.14 & 23.71 & 42.29 & \cellcolor{PaleBlue}\textbf{47.14} & 53.14 & 40.86 & 55.71 & \cellcolor{PaleBlue}\textbf{57.14} \\ 
\#2 & 35.71 & 27.43 & 45.43 & \cellcolor{PaleBlue}\textbf{51.71} & 58.86 & 46.86 & 62.57 & \cellcolor{PaleBlue}\textbf{62.57} \\
\#3 & 32.29 & 26.00 & 43.43 & \cellcolor{PaleBlue}\textbf{48.86} & 58.86 & 47.71 & 60.57 & \cellcolor{PaleBlue}\textbf{62.00} \\ 
\#4 & 33.14 & 20.29 & 42.29 & \cellcolor{PaleBlue}\textbf{44.86} & 55.71 & 42.86 & 57.14 & \cellcolor{PaleBlue}\textbf{56.57} \\ 
\#5 & 42.86 & 29.71 & 52.57 & \cellcolor{PaleBlue}\textbf{57.43} & 62.57 & 52.29 & 65.71 & \cellcolor{PaleBlue}\textbf{65.43} \\ 
\midrule
Overall & 35.83 & 25.43 & 45.20 & \cellcolor{PaleBlue}\textbf{50.00} & 57.83 & 46.12 & 60.34 & \cellcolor{PaleBlue}\textbf{60.74} \\
\toprule
\multirow{2}{*} {} & \multicolumn{4}{c}{Top1 IoU} & \multicolumn{4}{c}{Top3 IoU} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\ 
\midrule
\#1 & 0.31 & 0.18 & 0.36 & \cellcolor{PaleBlue}\textbf{0.42} & 0.50 & 0.39 & 0.51 & \cellcolor{PaleBlue}\textbf{0.53} \\ 
\#2 & 0.31 & 0.22 & 0.38 & \cellcolor{PaleBlue}\textbf{0.44} & 0.53 & 0.43 & 0.55 & \cellcolor{PaleBlue}\textbf{0.56} \\
\#3 & 0.29 & 0.21 & 0.37 & \cellcolor{PaleBlue}\textbf{0.43} & 0.52 & 0.43 & 0.54 & \cellcolor{PaleBlue}\textbf{0.56} \\ 
\#4 & 0.30 & 0.17 & 0.36 & \cellcolor{PaleBlue}\textbf{0.40} & 0.51 & 0.39 & 0.52 & \cellcolor{PaleBlue}\textbf{0.52} \\ 
\#5 & 0.38 & 0.24 & 0.44 & \cellcolor{PaleBlue}\textbf{0.50} & 0.57 & 0.47 & 0.59 & \cellcolor{PaleBlue}\textbf{0.60} \\ 
\midrule
Overall & 0.32 & 0.20 & 0.38 & \cellcolor{PaleBlue}\textbf{0.44} & 0.53 & 0.42 & 0.54 & \cellcolor{PaleBlue}\textbf{0.56} \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison against five different varied open-vocabulary sets}
\label{tab:table2}
\end{minipage}%
\hspace{0.5cm}   
\begin{minipage}{.45\linewidth}
\centering
\scalebox{0.40}{
\begin{tabular}{>{\centering\arraybackslash}m{2.5cm}cccccccc}
\toprule
\multirow{2}{*}{Relationship Set} & \multicolumn{4}{c}{Top1 Match Rate} & \multicolumn{4}{c}{Top3 Match Rate} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\  
\midrule
\#1 & 35.14 & 19.50 & 36.00 & \cellcolor{PaleBlue}\textbf{41.38} & 54.12 & 40.88 & 53.88 & \cellcolor{PaleBlue}\textbf{58.12} \\ 
\#2 & 35.71 & 21.50 & 36.75 & \cellcolor{PaleBlue}\textbf{44.62} & 59.12 & 47.62 & 62.38 & \cellcolor{PaleBlue}\textbf{62.88} \\
\#3 & 32.29 & 23.25 & 38.25 & \cellcolor{PaleBlue}\textbf{42.12} & 58.88 & 49.88 & 61.12 & \cellcolor{PaleBlue}\textbf{59.88} \\ 
\#4 & 33.14 & 18.75 & 36.50 & \cellcolor{PaleBlue}\textbf{40.38} & 56.38 & 43.12 & 55.38 & \cellcolor{PaleBlue}\textbf{56.38} \\ 
\#5 & 42.86 & 22.75 & 43.25 & \cellcolor{PaleBlue}\textbf{47.88} & 62.38 & 52.38 & 65.12 & \cellcolor{PaleBlue}\textbf{65.38} \\ 
\midrule
Overall & 35.83 & 21.15 & 38.15 & \cellcolor{PaleBlue}\textbf{43.28} & 58.18 & 46.76 & 59.58 & \cellcolor{PaleBlue}\textbf{60.53} \\
\toprule
\multirow{2}{*}{} & \multicolumn{4}{c}{Top1 IoU} & \multicolumn{4}{c}{Top3 IoU} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\  
\midrule
\#1 & 0.30 & 0.17 & 0.31 & \cellcolor{PaleBlue}\textbf{0.36} & 0.50 & 0.38 & 0.48 & \cellcolor{PaleBlue}\textbf{0.53} \\ 
\#2 & 0.30 & 0.19 & 0.32 & \cellcolor{PaleBlue}\textbf{0.39} & 0.54 & 0.43 & 0.55 & \cellcolor{PaleBlue}\textbf{0.56} \\
\#3 & 0.29 & 0.20 & 0.33 & \cellcolor{PaleBlue}\textbf{0.38} & 0.53 & 0.45 & 0.54 & \cellcolor{PaleBlue}\textbf{0.54} \\ 
\#4 & 0.30 & 0.16 & 0.30 & \cellcolor{PaleBlue}\textbf{0.36} & 0.52 & 0.40 & 0.50 & \cellcolor{PaleBlue}\textbf{0.52} \\ 
\#5 & 0.38 & 0.20 & 0.37 & \cellcolor{PaleBlue}\textbf{0.42} & 0.57 & 0.48 & 0.58 & \cellcolor{PaleBlue}\textbf{0.60} \\ 
\midrule
Overall & 0.32 & 0.18 & 0.33 & \cellcolor{PaleBlue}\textbf{0.38} & 0.53 & 0.43 & 0.53 & \cellcolor{PaleBlue}\textbf{0.55} \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison against five different varied relationship sets}
\label{tab:table3}
\end{minipage}
\end{table}
\subsection{Open-vocabulary Analysis}
Having presented insights on our system's performance on natural language queries for DOVE-G (as shown in Table~\ref{tab:table1}), we proceed to deepen our investigation into the system's resilience across diverse query sets. To accomplish this, we instead average the results from all scenes for each of the five vocabulary sets (refer to Table~\ref{tab:table2}). By doing so, we aim to provide a robust evaluation of our system's performance across a variety of query structures and word choices, simulating the varied ways in which users may interact with our system. In addition to experimenting with object vocabulary variations (a `coffee maker' to `espresso machine' or `coffee brewer'), and altering the order of entity referencing in the query, we also studied the impact of changing relationship vocabulary. In this experimental setup, the LLM is not bound to map relationships to a pre-determined set as before. Instead, the graph-based query contains a variety of relationship vocabulary. To illustrate, consider the queries ``A is to the left back corner of B" and ``A is behind and left to B". Previously, these relationships would map to a fixed relation like `left and behind'. Now, `front and left' as interpreted by the LLM can variate to `leftward and ahead', `northwest direction', or `towards the front and left', offering a broader range of relationship descriptions.  The evaluation results for these query sets are presented in Table~\ref{tab:table3}. 

\textbf{Varying object names}
Across all evaluated vocabulary sets, OVSG-L demonstrates the highest Top1 and Top3 match rates, outperforming the remaining methods. This pattern also persists for scores in the IoU category. 
Notably, OVSG-L's match rates span from 44.86\% to 57.43\% for Top1, and 56.57\% to 65.43\% for Top3.
Other methods, including OVIR-3D, OVSG-J, and OVSG-S, also exhibit robust performance, albeit lower than OVSG-L. All in all, contextual understanding of the target again proves to improve results from 35.83\% (OVIR-3D) to 50\% (OVSG-L) for top 1 match rate and 0.32 to 0.44 for the top 1 IoU. 

\textbf{Varying relationships} 
Compared to Table~\ref{tab:table2}, we observe a noticeable decrease in performance for the methods under the OVSG framework. This is likely due to the increased complexity introduced by the varied word choices for edges (relationships) in the sub-graph being matched. Despite this, two of the OVSG methods still outperform the OVIR-3D method, with the OVSG-L method delivering the strongest results.

\subsection{Robot application: Manipulation}
In order to exemplify the utility of OVSG in real-world manipulation scenarios, we devised a complex pick-and-place experiment. In this task, the robot is instructed to select one building block and position it on another. The complexity of the task stems from the multitude of blocks that are identical in both shape and color, necessitating the use of spatial context for differentiation. We formulated nine distinct tasks for this purpose (please refer to Appendix.~\ref{manip_exp_setup} for detailed setup). The effectiveness of the manipulation task was evaluated by comparing the success rate achieved by OVIR-3D and our newly proposed OVSG-L. The outcome of this comparative study is depicted in the accompanying table. The results demonstrate that our innovative OVSG-L model significantly enhances the object grounding accuracy in manipulation tasks involving a high prevalence of identical objects. This improvement highlights the potential of OVSG-L in complex manipulation scenarios, paving the way for further exploration in the field of robotics.

\subsection{Robot application: Navigation} We conducted a system test on a ROSMASTER R2 Ackermann Steering Robot for an object navigation task. The detailed setup can be found in Appendix.~\ref{nav_exp_setup}. We provided queries for seven different objects within a lab scene, using three slightly different languages to specify each object. These queries were then inputted into OVSG, and the grounded positions of the entities were returned to the robot. We considered the task successful if the robot's final position was within 1 meter of the queried objects. The results are presented in Table.~\ref{obj_nav}. From the table, it is evident that the proposed method successfully located the majority of user queries. However, there was one query that was not successfully located: ``The cloth on a chair in the office." In this case, we found OVIR-3D incorrectly recognized the cloth as part of a chair, resulting in the failure to locate it.

\begin{table}[htbp]
\centering
\begin{minipage}{.45\linewidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
object       & shoe  & bottle & chair & trash can\#1 & trash can\#2 & drawer & cloth \\ \midrule
success rate \% & 100.0 & 100.0  & 100.0  & 100.0      & 100.0       & 100.0  & 0.0   \\ \bottomrule
\end{tabular}%
}
\caption{Success rate of object navigation task}
\label{tab:obj_nav_result}
\end{minipage}%
\hspace{0.5cm}   
\begin{minipage}{.45\linewidth}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
object       & shoe  & bottle & chair & trash can\#1 & trash can\#2 & drawer & cloth \\ \midrule
success rate \% & 100.0 & 100.0  & 100.0  & 100.0      & 100.0       & 100.0  & 0.0   \\ \bottomrule
\end{tabular}%
}
\caption{Success rate of object navigation task}
\label{tab:obj_nav_result}
\end{minipage}%
\end{table}

==> Sections/doveg.tex <==

//////////////////////////////////User Status:  with_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.21
IoU_15:  30.75 %
IoU_25:  30.75 %
IoU_50:  25.25 %
IoU_75:  12.5 %
mAcc:  23.0
acc_15:  5
acc_25:  4
acc_50:  0
acc_75:  0
[Top3]mAcc:  41.0
[Top3]acc_15:  8
[Top3]acc_25:  7
[Top3]acc_50:  2
[Top3]acc_75:  1
num_queries:  400
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.365
IoU_15:  57.5 %
IoU_25:  55.25 %
IoU_50:  41.5 %
IoU_75:  16.25 %
mAcc:  35.5
acc_15:  8
acc_25:  7
acc_50:  1
acc_75:  0
[Top3]mAcc:  56.0
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  4
[Top3]acc_75:  2
num_queries:  400
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.425
IoU_15:  63.25 %
IoU_25:  61.0 %
IoU_50:  50.25 %
IoU_75:  25.0 %
mAcc:  44.8
acc_15:  8
acc_25:  8
acc_50:  2
acc_75:  0
[Top3]mAcc:  56.8
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  4
[Top3]acc_75:  2
num_queries:  400
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.545
IoU_15:  80.75 %
IoU_25:  78.5 %
IoU_50:  65.75 %
IoU_75:  32.25 %
mAcc:  54.2
acc_15:  8
acc_25:  8
acc_50:  3
acc_75:  2
[Top3]mAcc:  57.0
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  4
[Top3]acc_75:  2
num_queries:  400
********************************************************
//////////////////////////////////User Status:  no_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.14
IoU_15:  21.25 %
IoU_25:  21.25 %
IoU_50:  18.44 %
IoU_75:  5.62 %
mAcc:  13.8
acc_15:  2
acc_25:  1
acc_50:  0
acc_75:  0
[Top3]mAcc:  34.1
[Top3]acc_15:  6
[Top3]acc_25:  5
[Top3]acc_50:  1
[Top3]acc_75:  1
num_queries:  320
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.406
IoU_15:  63.12 %
IoU_25:  61.56 %
IoU_50:  49.69 %
IoU_75:  18.12 %
mAcc:  36.6
acc_15:  8
acc_25:  5
acc_50:  1
acc_75:  0
[Top3]mAcc:  58.1
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  5
[Top3]acc_75:  2
num_queries:  320
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.43
IoU_15:  65.94 %
IoU_25:  64.38 %
IoU_50:  53.12 %
IoU_75:  20.31 %
mAcc:  39.1
acc_15:  8
acc_25:  6
acc_50:  1
acc_75:  1
[Top3]mAcc:  56.2
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  5
[Top3]acc_75:  2
num_queries:  320
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.544
IoU_15:  81.56 %
IoU_25:  80.0 %
IoU_50:  67.81 %
IoU_75:  28.75 %
mAcc:  48.4
acc_15:  8
acc_25:  6
acc_50:  2
acc_75:  2
[Top3]mAcc:  56.6
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  5
[Top3]acc_75:  2
num_queries:  320
********************************************************
//////////////////////////////////User Status:  with_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.21
IoU_15:  123
IoU_25:  123
IoU_50:  101
IoU_75:  50
mAcc:  23.0
acc_15:  5
acc_25:  4
acc_50:  0
acc_75:  0
[Top3]mAcc:  41.0253
[Top3]acc_15:  8
[Top3]acc_25:  7
[Top3]acc_50:  2
[Top3]acc_75:  1
num_queries:  400
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.365
IoU_15:  230
IoU_25:  221
IoU_50:  166
IoU_75:  65
mAcc:  35.5
acc_15:  8
acc_25:  7
acc_50:  1
acc_75:  0
[Top3]mAcc:  56.0
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  4
[Top3]acc_75:  2
num_queries:  400
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.425
IoU_15:  253
IoU_25:  244
IoU_50:  201
IoU_75:  100
mAcc:  44.8
acc_15:  8
acc_25:  8
acc_50:  2
acc_75:  0
[Top3]mAcc:  56.8
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  4
[Top3]acc_75:  2
num_queries:  400
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.545
IoU_15:  323
IoU_25:  314
IoU_50:  263
IoU_75:  129
mAcc:  54.2
acc_15:  8
acc_25:  8
acc_50:  3
acc_75:  2
[Top3]mAcc:  57.0
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  4
[Top3]acc_75:  2
num_queries:  400
********************************************************

//////////////////////////////////User Status:  no_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.14
IoU_15:  68
IoU_25:  68
IoU_50:  59
IoU_75:  18
mAcc:  13.8
acc_15:  2
acc_25:  1
acc_50:  0
acc_75:  0
[Top3]mAcc:  34.1
[Top3]acc_15:  6
[Top3]acc_25:  5
[Top3]acc_50:  1
[Top3]acc_75:  1
num_queries:  320
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.406
IoU_15:  202
IoU_25:  197
IoU_50:  159
IoU_75:  58
mAcc:  36.6
acc_15:  8
acc_25:  5
acc_50:  1
acc_75:  0
[Top3]mAcc:  58.1
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  5
[Top3]acc_75:  2
num_queries:  320
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.43
IoU_15:  211
IoU_25:  206
IoU_50:  170
IoU_75:  65
mAcc:  39.1
acc_15:  8
acc_25:  6
acc_50:  1
acc_75:  1
[Top3]mAcc:  56.2
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  5
[Top3]acc_75:  2
num_queries:  320
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.544
IoU_15:  261
IoU_25:  256
IoU_50:  217
IoU_75:  92
mAcc:  48.4
acc_15:  8
acc_25:  6
acc_50:  2
acc_75:  2
[Top3]mAcc:  56.6
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  5
[Top3]acc_75:  2
num_queries:  320
********************************************************

==> Sections/icl.tex <==
//////////////////////////////////User Status:  no_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.194
IoU_15:  33.16 %
IoU_25:  32.11 %
IoU_50:  22.63 %
IoU_75:  3.16 %
mAcc:  16.8
acc_15:  4
acc_25:  2
acc_50:  0
acc_75:  0
[Top3]mAcc:  48.9
[Top3]acc_15:  8
[Top3]acc_25:  6
[Top3]acc_50:  4
[Top3]acc_75:  0
num_queries:  190
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.365
IoU_15:  56.84 %
IoU_25:  56.84 %
IoU_50:  48.95 %
IoU_75:  10.0 %
mAcc:  35.3
acc_15:  6
acc_25:  5
acc_50:  2
acc_75:  0
[Top3]mAcc:  54.7
[Top3]acc_15:  8
[Top3]acc_25:  6
[Top3]acc_50:  5
[Top3]acc_75:  1
num_queries:  190
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.408
IoU_15:  65.79 %
IoU_25:  64.21 %
IoU_50:  51.58 %
IoU_75:  13.68 %
mAcc:  38.9
acc_15:  6
acc_25:  5
acc_50:  3
acc_75:  0
[Top3]mAcc:  54.7
[Top3]acc_15:  8
[Top3]acc_25:  6
[Top3]acc_50:  5
[Top3]acc_75:  2
num_queries:  190
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.564
IoU_15:  89.47 %
IoU_25:  87.89 %
IoU_50:  68.95 %
IoU_75:  22.63 %
mAcc:  51.6
acc_15:  8
acc_25:  6
acc_50:  4
acc_75:  2
[Top3]mAcc:  55.8
[Top3]acc_15:  8
[Top3]acc_25:  6
[Top3]acc_50:  5
[Top3]acc_75:  2
num_queries:  190
********************************************************
//////////////////////////////////User Status:  with_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.35
IoU_15:  51.25 %
IoU_25:  49.86 %
IoU_50:  44.29 %
IoU_75:  16.43 %
mAcc:  44.3
acc_15:  8
acc_25:  8
acc_50:  2
acc_75:  0
[Top3]mAcc:  66.3
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  6
[Top3]acc_75:  2
num_queries:  359
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.348
IoU_15:  52.65 %
IoU_25:  52.65 %
IoU_50:  45.96 %
IoU_75:  11.14 %
mAcc:  39.3
acc_15:  8
acc_25:  7
acc_50:  2
acc_75:  0
[Top3]mAcc:  72.4
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  7
[Top3]acc_75:  3
num_queries:  359
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.489
IoU_15:  72.98 %
IoU_25:  71.87 %
IoU_50:  61.84 %
IoU_75:  22.56 %
mAcc:  59.6
acc_15:  8
acc_25:  8
acc_50:  5
acc_75:  1
[Top3]mAcc:  74.1
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  7
[Top3]acc_75:  4
num_queries:  359
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.635
IoU_15:  93.87 %
IoU_25:  92.76 %
IoU_50:  78.55 %
IoU_75:  32.31 %
mAcc:  74.1
acc_15:  8
acc_25:  8
acc_50:  7
acc_75:  4
[Top3]mAcc:  74.7
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  7
[Top3]acc_75:  4
num_queries:  359
********************************************************
//////////////////////////////////User Status:  with_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.35
IoU_15:  184
IoU_25:  179
IoU_50:  159
IoU_75:  59
mAcc:  44.3
acc_15:  8
acc_25:  8
acc_50:  2
acc_75:  0
[Top3]mAcc:  66.3
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  6
[Top3]acc_75:  2
num_queries:  359
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.348
IoU_15:  189
IoU_25:  189
IoU_50:  165
IoU_75:  40
mAcc:  39.3
acc_15:  8
acc_25:  7
acc_50:  2
acc_75:  0
[Top3]mAcc:  72.4
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  7
[Top3]acc_75:  3
num_queries:  359
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.489
IoU_15:  262
IoU_25:  258
IoU_50:  222
IoU_75:  81
mAcc:  59.6
acc_15:  8
acc_25:  8
acc_50:  5
acc_75:  1
[Top3]mAcc:  74.1
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  7
[Top3]acc_75:  4
num_queries:  359
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.635
IoU_15:  337
IoU_25:  333
IoU_50:  282
IoU_75:  116
mAcc:  74.1
acc_15:  8
acc_25:  8
acc_50:  7
acc_75:  4
[Top3]mAcc:  74.7
[Top3]acc_15:  8
[Top3]acc_25:  8
[Top3]acc_50:  7
[Top3]acc_75:  4
num_queries:  359
********************************************************

//////////////////////////////////User Status:  no_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.194
IoU_15:  63
IoU_25:  61
IoU_50:  43
IoU_75:  6
mAcc:  16.8
acc_15:  4
acc_25:  2
acc_50:  0
acc_75:  0
[Top3]mAcc:  48.9
[Top3]acc_15:  8
[Top3]acc_25:  6
[Top3]acc_50:  4
[Top3]acc_75:  0
num_queries:  190
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.365
IoU_15:  108
IoU_25:  108
IoU_50:  93
IoU_75:  19
mAcc:  35.3
acc_15:  6
acc_25:  5
acc_50:  2
acc_75:  0
[Top3]mAcc:  54.7
[Top3]acc_15:  8
[Top3]acc_25:  6
[Top3]acc_50:  5
[Top3]acc_75:  1
num_queries:  190
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.408
IoU_15:  125
IoU_25:  122
IoU_50:  98
IoU_75:  26
mAcc:  38.9
acc_15:  6
acc_25:  5
acc_50:  3
acc_75:  0
[Top3]mAcc:  54.7
[Top3]acc_15:  8
[Top3]acc_25:  6
[Top3]acc_50:  5
[Top3]acc_75:  2
num_queries:  190
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.564
IoU_15:  170
IoU_25:  167
IoU_50:  131
IoU_75:  43
mAcc:  51.6
acc_15:  8
acc_25:  6
acc_50:  4
acc_75:  2
[Top3]mAcc:  55.8
[Top3]acc_15:  8
[Top3]acc_25:  6
[Top3]acc_50:  5
[Top3]acc_75:  2
num_queries:  190
********************************************************



==> Sections/scannet.tex <==
//////////////////////////////////User Status:  with_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.216
IoU_15:  32.78 %
IoU_25:  30.91 %
IoU_50:  24.83 %
IoU_75:  12.38 %
mAcc:  24.3
acc_15:  250
acc_25:  131
acc_50:  12
acc_75:  1
[Top3]mAcc:  47.8
[Top3]acc_15:  303
[Top3]acc_25:  284
[Top3]acc_50:  138
[Top3]acc_75:  19
num_queries:  20173
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.376
IoU_15:  57.57 %
IoU_25:  54.27 %
IoU_50:  43.86 %
IoU_75:  20.92 %
mAcc:  38.6
acc_15:  290
acc_25:  252
acc_50:  61
acc_75:  8
[Top3]mAcc:  56.3
[Top3]acc_15:  306
[Top3]acc_25:  302
[Top3]acc_50:  203
[Top3]acc_75:  39
num_queries:  20173
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.435
IoU_15:  65.57 %
IoU_25:  62.49 %
IoU_50:  51.21 %
IoU_75:  24.74 %
mAcc:  47.8
acc_15:  306
acc_25:  291
acc_50:  141
acc_75:  16
[Top3]mAcc:  59.9
[Top3]acc_15:  309
[Top3]acc_25:  304
[Top3]acc_50:  227
[Top3]acc_75:  59
num_queries:  20173
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.548
IoU_15:  83.77 %
IoU_25:  79.22 %
IoU_50:  63.88 %
IoU_75:  30.57 %
mAcc:  58.8
acc_15:  308
acc_25:  302
acc_50:  217
acc_75:  62
[Top3]mAcc:  61.6
[Top3]acc_15:  309
[Top3]acc_25:  304
[Top3]acc_50:  233
[Top3]acc_75:  70
num_queries:  20173
********************************************************
//////////////////////////////////User Status:  no_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.156
IoU_15:  24.77 %
IoU_25:  22.68 %
IoU_50:  17.22 %
IoU_75:  8.03 %
mAcc:  15.3
acc_15:  138
acc_25:  48
acc_50:  4
acc_75:  0
[Top3]mAcc:  41.2
[Top3]acc_15:  286
[Top3]acc_25:  256
[Top3]acc_50:  83
[Top3]acc_75:  12
num_queries:  18683
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.389
IoU_15:  59.94 %
IoU_25:  56.45 %
IoU_50:  45.13 %
IoU_75:  21.05 %
mAcc:  38.5
acc_15:  287
acc_25:  251
acc_50:  65
acc_75:  8
[Top3]mAcc:  52.9
[Top3]acc_15:  304
[Top3]acc_25:  294
[Top3]acc_50:  167
[Top3]acc_75:  35
num_queries:  18683
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.413
IoU_15:  63.97 %
IoU_25:  60.05 %
IoU_50:  47.79 %
IoU_75:  22.11 %
mAcc:  41.0
acc_15:  288
acc_25:  266
acc_50:  75
acc_75:  12
[Top3]mAcc:  53.6
[Top3]acc_15:  303
[Top3]acc_25:  296
[Top3]acc_50:  173
[Top3]acc_75:  34
num_queries:  18683
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.525
IoU_15:  81.88 %
IoU_25:  76.87 %
IoU_50:  60.34 %
IoU_75:  27.78 %
mAcc:  52.2
acc_15:  304
acc_25:  292
acc_50:  164
acc_75:  34
[Top3]mAcc:  56.3
[Top3]acc_15:  307
[Top3]acc_25:  301
[Top3]acc_50:  194
[Top3]acc_75:  45
num_queries:  18683
********************************************************
//////////////////////////////////User Status:  no_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.156
IoU_15:  4627
IoU_25:  4237
IoU_50:  3217
IoU_75:  1501
mAcc:  15.3
acc_15:  138
acc_25:  48
acc_50:  4
acc_75:  0
[Top3]mAcc:  41.2
[Top3]acc_15:  286
[Top3]acc_25:  256
[Top3]acc_50:  83
[Top3]acc_75:  12
num_queries:  18683
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.389
IoU_15:  11198
IoU_25:  10546
IoU_50:  8431
IoU_75:  3932
mAcc:  38.5
acc_15:  287
acc_25:  251
acc_50:  65
acc_75:  8
[Top3]mAcc:  52.9
[Top3]acc_15:  304
[Top3]acc_25:  294
[Top3]acc_50:  167
[Top3]acc_75:  35
num_queries:  18683
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.413
IoU_15:  11951
IoU_25:  11220
IoU_50:  8928
IoU_75:  4130
mAcc:  41.0
acc_15:  288
acc_25:  266
acc_50:  75
acc_75:  12
[Top3]mAcc:  53.6
[Top3]acc_15:  303
[Top3]acc_25:  296
[Top3]acc_50:  173
[Top3]acc_75:  34
num_queries:  18683
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.525
IoU_15:  15297
IoU_25:  14361
IoU_50:  11274
IoU_75:  5191
mAcc:  52.2
acc_15:  304
acc_25:  292
acc_50:  164
acc_75:  34
[Top3]mAcc:  56.3
[Top3]acc_15:  307
[Top3]acc_25:  301
[Top3]acc_50:  194
[Top3]acc_75:  45
num_queries:  18683
********************************************************
//////////////////////////////////User Status:  with_user //////////////////////////////////
***************************Method:  jaccard ***************************
mIoU_3d:  0.216
IoU_15:  6613
IoU_25:  6235
IoU_50:  5008
IoU_75:  2498
mAcc:  24.3
acc_15:  250
acc_25:  131
acc_50:  12
acc_75:  1
[Top3]mAcc:  47.8
[Top3]acc_15:  303
[Top3]acc_25:  284
[Top3]acc_50:  138
[Top3]acc_75:  19
num_queries:  20173
********************************************************

***************************Method:  base ***************************
mIoU_3d:  0.376
IoU_15:  11614
IoU_25:  10947
IoU_50:  8847
IoU_75:  4221
mAcc:  38.6
acc_15:  290
acc_25:  252
acc_50:  61
acc_75:  8
[Top3]mAcc:  56.3
[Top3]acc_15:  306
[Top3]acc_25:  302
[Top3]acc_50:  203
[Top3]acc_75:  39
num_queries:  20173
********************************************************

***************************Method:  szymkiewicz_simpson ***************************
mIoU_3d:  0.435
IoU_15:  13227
IoU_25:  12606
IoU_50:  10331
IoU_75:  4990
mAcc:  47.8
acc_15:  306
acc_25:  291
acc_50:  141
acc_75:  16
[Top3]mAcc:  59.9
[Top3]acc_15:  309
[Top3]acc_25:  304
[Top3]acc_50:  227
[Top3]acc_75:  59
num_queries:  20173
********************************************************

***************************Method:  prob ***************************
mIoU_3d:  0.548
IoU_15:  16898
IoU_25:  15982
IoU_50:  12886
IoU_75:  6166
mAcc:  58.8
acc_15:  308
acc_25:  302
acc_50:  217
acc_75:  62
[Top3]mAcc:  61.6
[Top3]acc_15:  309
[Top3]acc_25:  304
[Top3]acc_50:  233
[Top3]acc_75:  70
num_queries:  20173
********************************************************

==> Sections/tables.tex <==
\begin{table}[htbp]
\centering
\scalebox{0.8}{
\begin{tabular}{>{\centering\arraybackslash}m{2.5cm}c>{\centering\arraybackslash}m{1.5cm}cccccccc}
\toprule
\multirow{2}{*}{ScanNet} & \multirow{2}{*}{Num of queries} & \multicolumn{4}{c}{Top1 Match Rate} & \multicolumn{4}{c}{Top3 Match Rate} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
& & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\ 
\midrule
Without Users & 18,863 & 38.5 & 15.3 & 41.0 & \cellcolor{PaleBlue}\textbf{52.2} & 52.9 & 41.2 & 53.6 & \cellcolor{PaleBlue}\textbf{56.3} \\
With Users & 20,173 & 38.6 & 24.3 & 47.8 & \cellcolor{PaleBlue}\textbf{58.8} & 56.3 & 47.8 & 59.9 & \cellcolor{PaleBlue}\textbf{61.6} \\
\toprule
\multirow{2}{*} {DOVE-G} & \multirow{2}{*}{Num of queries} & \multicolumn{4}{c}{Top1 Match Rate} & \multicolumn{4}{c}{Top3 Match Rate} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
& & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\ 
\midrule
Without Users & 320 & 36.6 & 13.8 & 39.1 & \cellcolor{PaleBlue}\textbf{48.4} & 58.1 & 34.1 & 56.2 & \cellcolor{PaleBlue}\textbf{56.6} \\
With Users & 400 & 35.5 & 23.0 & 44.8 & \cellcolor{PaleBlue}\textbf{54.2} & 56.0 & 41.0 & 56.8 & \cellcolor{PaleBlue}\textbf{57.0} \\
\toprule
\multirow{2}{*} {ICL-NUIM} & \multirow{2}{*}{Num of queries} & \multicolumn{4}{c}{Top1 Match Rate} & \multicolumn{4}{c}{Top3 Match Rate} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
& & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\ 
\midrule
Without Users & 190 & 35.3 & 16.8 & 38.9 & \cellcolor{PaleBlue}\textbf{51.6} & 54.7 & 48.9 & 54.7 & \cellcolor{PaleBlue}\textbf{55.8} \\
With Users & 359 & 39.3 & 44.3 & 59.6 & \cellcolor{PaleBlue}\textbf{74.1} & 72.4 & 66.3 & 74.1 & \cellcolor{PaleBlue}\textbf{74.7} \\

\bottomrule
\end{tabular}
}
\caption{Grounding match rates averaged over all queries in ScanNet, DOVE-G, and ICL-NUIM datasets}
\label{tab:add1}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ScanNet(w/o users)  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
OVIR-3D & 0.389 & 59.94\%  & 56.45\%  & 45.13\%      & 21.05\%     \\ \midrule
OVSG-J & 0.156 & 24.77\%  & 22.68\%  & 17.22\%      & 8.03\%     \\ \midrule
OVSG-S & 0.413 & 63.97\%  & 60.05\%  & 47.79\%      & 22.11\%     \\ \midrule
OVSG-L & 0.525 & 81.88\%  & 76.87\%  & 60.34\%      & 27.78\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average 3D IoU scores on the ScanNet dataset for 18,683 queries w/o users}
\label{tab:add2}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ScanNet(w/o users)  & $mAcc^{1}$\  & $Acc^{1}_{15}$ & $Acc^{1}_{25}$ & $Acc^{1}_{50}$ & $Acc^{1}_{75}$  \\ \midrule
OVIR-3D & 38.725\% & 91.99\%  & 80.45\%  & 20.83\%      & 2.56\%     \\ \midrule
OVSG-J & 14.85\% & 44.23\%  & 15.38\%  & 1.28\%      & 0.0\%     \\ \midrule
OVSG-S & 40.772\% & 92.31\%  & 85.26\%  & 24.04\%      & 3.85\%     \\ \midrule
OVSG-L & 52.881\% & 97.44\%  & 93.59\%  & 52.56\%      & 10.9\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average top1 grounding accuracy scores on the ScanNet dataset for 18,683 queries w/o users}
\label{tab:add3}
\end{table}
\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ScanNet(w/o users)  & $mAcc^{3}$\  & $Acc^{3}_{15}$ & $Acc^{3}_{25}$ & $Acc^{3}_{50}$ & $Acc^{3}_{75}$  \\ \midrule
OVIR-3D & 53.326\% & 97.44\%  & 94.23\%  & 53.53\%      & 11.22\%     \\ \midrule
OVSG-J & 40.676\% & 91.67\%  & 82.05\%  & 26.6\%      & 3.85\%     \\ \midrule
OVSG-S & 53.825\% & 97.12\%  & 94.87\%  & 55.45\%      & 10.9\%     \\ \midrule
OVSG-L & 56.678\% & 98.4\%  & 96.47\%  & 62.18\%      & 14.42\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average top3 grounding accuracy scores on the ScanNet dataset for 18,683 queries w/o users}
\label{tab:add4}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ScanNet(with users)  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
OVIR-3D & 0.366 & 58.25\%  & 53.75\%  & 42.5\%      & 19.25\%     \\ \midrule
OVSG-J & 0.216 & 32.78\%  & 30.91\%  & 24.83\%      & 12.38\%     \\ \midrule
OVSG-S & 0.429 & 65.0\%  & 60.5\%  & 51.25\%      & 27.5\%     \\ \midrule
OVSG-L & 0.527 & 78.75\%  & 74.25\%  & 63.75\%      & 35.0\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average 3D IoU scores on the ScanNet dataset for 20,713 queries with users}
\label{tab:add5}
\end{table}
\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ScanNet(with users)  & $mAcc^{1}$\  & $Acc^{1}_{15}$ & $Acc^{1}_{25}$ & $Acc^{1}_{50}$ & $Acc^{1}_{75}$  \\ \midrule
OVIR-3D & 37.83\% & 92.95\%  & 80.77\%  & 19.55\%      & 2.56\%     \\ \midrule
OVSG-J & 24.335\% & 65.93\%  & 21.32\%  & 1.49\%      & 0.0\%     \\ \midrule
OVSG-S & 47.914\% & 98.08\%  & 93.27\%  & 45.19\%      & 5.13\%     \\ \midrule
OVSG-L & 59.644\% & 98.72\%  & 96.79\%  & 69.55\%      & 19.87\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average top1 grounding accuracy scores on the ScanNet dataset for 20,713 queries with users}
\label{tab:add6}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ScanNet(with users)  & $mAcc^{3}$\  & $Acc^{3}_{15}$ & $Acc^{3}_{25}$ & $Acc^{3}_{50}$ & $Acc^{3}_{75}$  \\ \midrule
OVIR-3D & 55.986\% & 98.08\%  & 96.79\%  & 65.06\%      & 12.5\%     \\ \midrule
OVSG-J & 47.841\% & 97.12\%  & 91.03\%  & 44.23\%      & 6.09\%     \\ \midrule
OVSG-S & 60.271\% & 99.04\%  & 97.44\%  & 72.76\%      & 18.91\%     \\ \midrule
OVSG-L & 61.969\% & 99.04\%  & 97.44\%  & 74.68\%      & 22.44\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average top3 grounding accuracy scores on the ScanNet dataset for 20,713 queries with users}
\label{tab:add7}
\end{table}


\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ICL(with users)  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
OVIR-3D & 0.342 & 52.05\%  & 52.05\%  & 45.04\%      & 10.66\%     \\ \midrule
OVSG-J & 0.352 & 51.26\%  & 50.16\%  & 44.88\%      & 16.84\%     \\ \midrule
OVSG-S & 0.488 & 73.14\%  & 71.67\%  & 61.79\%      & 22.45\%     \\ \midrule
OVSG-L & 0.634 & 93.98\%  & 92.51\%  & 78.76\%      & 32.29\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average 3D IoU scores on the ICL-NUIM dataset for 359 queries with users}
\label{tab:add8}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ICL(with users)  & $mAcc^{1}$\  & $Acc^{1}_{15}$ & $Acc^{1}_{25}$ & $Acc^{1}_{50}$ & $Acc^{1}_{75}$  \\ \midrule
OVIR-3D & 38.519\% & 100.0\%  & 87.5\%  & 25.0\%      & 0.0\%     \\ \midrule
OVSG-J & 44.351\% & 100.0\%  & 100.0\%  & 25.0\%      & 0.0\%     \\ \midrule
OVSG-S & 58.895\% & 100.0\%  & 100.0\%  & 87.5\%      & 50.0\%     \\ \midrule
OVSG-L & 73.421\% & 100.0\%  & 100.0\%  & 87.5\%      & 50.0\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average top1 grounding accuracy scores on the ICL-NUIM dataset for 359 queries with users}
\label{tab:add9}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ICL(with users)  & $mAcc^{3}$\  & $Acc^{3}_{15}$ & $Acc^{3}_{25}$ & $Acc^{3}_{50}$ & $Acc^{3}_{75}$  \\ \midrule
OVIR-3D & 71.647\% & 100.0\%  & 100.0\%  & 87.5\%      & 37.5\%     \\ \midrule
OVSG-J & 65.753\% & 100.0\%  & 100.0\%  & 75.0\%      & 25.0\%     \\ \midrule
OVSG-S & 73.368\% & 100.0\%  & 100.0\%  & 87.5\%      & 50.0\%     \\ \midrule
OVSG-L & 73.884\% & 100.0\%  & 100.0\%  & 87.5\%      & 50.0\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average top3 grounding accuracy scores on the ICL-NUIM dataset for 359 queries with users}
\label{tab:add10}
\end{table}


\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ICL(w/o users)  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
ConceptFusion (w/o rel) & 0.083 & 15.89\%  & 7.44\%  & 0.0\%      & 0.0\%     \\ \midrule
ConceptFusion (w/o rel 190) & 0.078 & 16.45\%  & 5.0\%  & 0.0\%      & 0.0\%     \\ \midrule
ConceptFusion & 0.032 & 3.57\%  & 0.0\%  & 0.0\%      & 0.0\%     \\ \midrule
OVIR-3D & 0.357 & 56.41\%  & 56.41\%  & 45.44\%      & 10.48\%     \\ \midrule
OVSG-J & 0.181 & 30.43\%  & 29.53\%  & 21.48\%      & 3.63\%     \\ \midrule
OVSG-S & 0.406 & 66.26\%  & 64.05\%  & 49.06\%      & 14.61\%     \\ \midrule
OVSG-L & 0.566 & 90.48\%  & 88.28\%  & 67.03\%      & 24.33\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average 3D IoU scores on the ICL-NUIM dataset for 190 queries with users}
\label{tab:add8}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ICL(w/o users)  & $mAcc^{1}$\  & $Acc^{1}_{15}$ & $Acc^{1}_{25}$ & $Acc^{1}_{50}$ & $Acc^{1}_{75}$  \\ \midrule
OVIR-3D & 32.064\% & 75.0\%  & 62.5\%  & 25.0\%      & 0.0\%     \\ \midrule
OVSG-J & 15.772\% & 50.0\%  & 25.0\%  & 0.0\%      & 0.0\%     \\ \midrule
OVSG-S & 36.287\% & 75.0\%  & 62.5\%  & 37.5\%      & 0.0\%     \\ \midrule
OVSG-L & 49.462\% & 100.0\%  & 75.0\%  & 50.0\%      & 25.0\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average top1 grounding accuracy scores on the ICL-NUIM dataset for 190 queries with users}
\label{tab:add9}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
ICL(w/o users)  & $mAcc^{3}$\  & $Acc^{3}_{15}$ & $Acc^{3}_{25}$ & $Acc^{3}_{50}$ & $Acc^{3}_{75}$  \\ \midrule
OVIR-3D & 51.32\% & 100.0\%  & 75.0\%  & 62.5\%      & 12.5\%     \\ \midrule
OVSG-J & 46.514\% & 100.0\%  & 75.0\%  & 50.0\%      & 0.0\%     \\ \midrule
OVSG-S & 52.007\% & 100.0\%  & 75.0\%  & 62.5\%      & 25.0\%     \\ \midrule
OVSG-L & 52.63\% & 100.0\%  & 75.0\%  & 62.5\%      & 25.0\%     \\ \bottomrule
\end{tabular}%
}
\caption{Average top3 grounding accuracy scores on the ICL-NUIM dataset for 190 queries with users}
\label{tab:add10}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
living\_room\_traj0\_frei\_png  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
ConceptFusion(w/o rel) & 22.1\% & 16  & 16  & 0      & 0     \\ \midrule
ConceptFusion & 5.2\% & 3  & 1  & 0      & 0    \\ \midrule
OVIR-3D & 34.2\% & 15  & 15  & 9      & 4      \\ \midrule
OVSG-J & 2.4\% & 1  & 1  & 1      & 0     \\ \midrule
OVSG-S & 38.4\% & 17  & 17  & 11      & 4     \\ \midrule
OVSG-L & 40.8\% & 18  & 18  & 12      & 4     \\ \bottomrule
\end{tabular}%
}
\caption{Grounding Accuracy of OVSG \& ConceptFusion on ICL-NUIM Living\_Room\_Trajectory0 for 26 queries without users}
\label{tab:add11}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
living\_room\_traj1\_frei\_png  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
ConceptFusion(w/o rel) & 29.5\% & 21  & 17  & 14      & 0     \\ \midrule
ConceptFusion & 14.5\% & 9 & 9 & 5 & 0     \\ \midrule
OVIR-3D & 44\% & 24  & 24  & 23      & 0     \\ \midrule
OVSG-J & 22.8\% & 13  & 13  & 10      & 0     \\ \midrule
OVSG-S & 35.3\% & 20  & 20  & 19      & 0     \\ \midrule
OVSG-L & 51.1\% & 27  & 27  & 24      & 5     \\ \bottomrule
\end{tabular}%
}
\caption{Grounding Accuracy of OVSG \& ConceptFusion on ICL-NUIM Living\_Room\_Trajectory1 for 34 queries without users}
\label{tab:add1}
\end{table}


\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
living\_room\_traj2\_frei\_png  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
ConceptFusion(w/o rel) & 16.6\% & 13  & 4  & 0     & 0    \\ \midrule
ConceptFusion & 3.1\% & 1  & 0  & 0  & 0    \\ \midrule
OVIR-3D & 36.6\% & 14  & 14  & 14      & 8    \\ \midrule
OVSG-J & 18\% & 12  & 10  & 1      & 0     \\ \midrule
OVSG-S & 50.2\% & 23  & 23  & 14      & 8     \\ \midrule
OVSG-L & 55.8\% & 26  & 26  & 15      & 8     \\ \bottomrule
\end{tabular}%
}
\caption{Grounding Accuracy of OVSG \& ConceptFusion on ICL-NUIM Living\_Room\_Trajectory2 for 28 queries without users}
\label{tab:add12}
\end{table}


\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
living\_room\_traj3\_frei\_png  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
ConceptFusion(w/o rel) & 8.5\% & 0  & 0 & 0      & 0     \\ \midrule
ConceptFusion & 8.1\% & 0  & 0 & 0    & 0    \\ \midrule
OVIR-3D & 6.3\% & 2  & 2  & 0     & 0     \\ \midrule
OVSG-J & 13.6\% & 4 & 4 & 4     & 0     \\ \midrule
OVSG-S & 19.2\% & 7  & 4  & 2     & 2     \\ \midrule
OVSG-L & 46.5\% & 14  & 11  & 9      & 5     \\ \bottomrule
\end{tabular}%
}
\caption{Grounding Accuracy of OVSG \& ConceptFusion on ICL-NUIM Living\_Room\_Trajectory3 for 17 queries without users}
\label{tab:add13}
\end{table}


\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
office\_room\_traj0\_frei\_png  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\% \\ \midrule
ConceptFusion(w/o rel) & 3.7\% & 0 & 0 & 0    & 0    \\ \midrule
ConceptFusion & 2.5\% & 0 & 0 & 0  & 0   \\ \midrule
OVIR-3D & 42.9\% & 19  & 19  & 19      & 0     \\ \midrule
OVSG-J & 26.8 & 13  & 13  & 12      & 0     \\ \midrule
OVSG-S & 42.9\% & 19  & 19  & 19      & 0     \\ \midrule
OVSG-L & 64\% & 29  & 29  & 28      & 0     \\ \bottomrule
\end{tabular}%
}
\caption{Grounding Accuracy of OVSG \& ConceptFusion on ICL-NUIM Office\_Room\_Trajectory0 for 29 queries without users}
\label{tab:add13}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
office\_room\_traj1\_frei\_png  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
ConceptFusion(w/o rel) & 2.4\% & 0 & 0 & 0    & 0    \\ \midrule
ConceptFusion & 1.8\% & 0  & 0  & 0     & 0    \\ \midrule
OVIR-3D & 49.1\% & 13  & 13  & 13      & 6    \\ \midrule
OVSG-J & 31.9\% & 8 & 8  & 8      & 4     \\ \midrule
OVSG-S & 53.7\% & 14  & 14  & 14      & 7     \\ \midrule
OVSG-L & 74\% & 19  & 19  & 18      & 11     \\ \bottomrule
\end{tabular}%
}
\caption{Grounding Accuracy of OVSG \& ConceptFusion on ICL-NUIM Office\_Room\_Trajectory1 for 19 queries without users}
\label{tab:add14}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
office\_room\_traj2\_frei\_png  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
ConceptFusion(w/o rel) & 2\% & 0  & 0  & 0      & 0     \\ \midrule
ConceptFusion & 0.9\% & 0  & 0 & 0     & 0     \\ \midrule
OVIR-3D & 44.2\% & 10  & 10 & 4  & 1    \\ \midrule
OVSG-J & 0.0\% & 0  & 0  & 0      & 0     \\ \midrule
OVSG-S & 44.2\% & 10  & 10  & 4      & 1     \\ \midrule
OVSG-L & 54.3\% & 12  & 12  & 5      & 2     \\ \bottomrule
\end{tabular}%
}
\caption{Grounding Accuracy of OVSG \& ConceptFusion on ICL-NUIM Office\_Room\_Trajectory2 for 12 queries without users}
\label{tab:add15}
\end{table}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
office\_room\_traj3\_frei\_png  & $mAcc_{G}$  & $Acc_{G} >$ 15\% & $Acc_{G} >$ 25\% & $Acc_{G} >$ 50\% & $Acc_{G} >$ 75\%  \\ \midrule
ConceptFusion(w/o rel) & 6.9\% & 3  & 0  & 0  & 0     \\ \midrule
ConceptFusion & 4.2\% & 0  & 0  & 0   & 0     \\ \midrule
OVIR-3D & 28\% & 11  & 11 & 11     & 0     \\ \midrule
OVSG-J & 29.2\% & 12 & 12  & 7      & 2     \\ \midrule
OVSG-S & 41\% & 15  & 15  & 15     & 4     \\ \midrule
OVSG-L & 66.1\% & 25 & 25  & 20      & 8     \\ \bottomrule
\end{tabular}%
}
\caption{Grounding Accuracy of OVSG \& ConceptFusion on ICL-NUIM Office\_Room\_Trajectory3 for 25 queries without users}
\label{tab:office_traj3_acc}
\end{table}


\textcolor{blue}{Object grounding diverges from object detection and segmentation tasks in its pursuit to localize an object within a 2D image or a 3D scene based on a textual descriptor. In 2D grounding, there is a rich tapestry of research, such as \cite{Findit}, that capitalizes on vision-language alignment techniques to bridge the gap between visual and linguistic representations. Venturing into the 3D domain, object grounding acquires added complexity due to its association with robot navigation challenges, thus garnering attention from the robotics community. A notable example is COWs~\cite{gadre2023cows}, which synergizes a CLIP gradient detector with a navigation policy, paving the way for adept zero-shot object grounding. In contrast, NLMaps~\cite{chen2023open} emphasizes integrating pixel-level open-vocabulary attributes into 3D scene reconstruction, culminating in a scene representation that can be probed with queries. When a query arises, NLMaps leverages a Large Language Model (LLM) to fragment the query into word-level units and then scours the scene representation for matches. This strategy of harnessing an LLM for query dissection echoes our methodology. However, NLMaps appears to sidestep the nuanced inter-relationships in their structural framework.}

\textcolor{blue}{Breaking away from the tradition of employing a singular encoder as observed in prior works like \cite{chen2023open, conceptfusion}, we adopt distinct encoders tailored to specific node and relationship types. Notably, the encoders for each graph, $G_s$ and $G_q$, are not identical, reflecting the unique inputs they process.

For $G_s$, object features are extracted by applying OVIR-3D to the scene's 3D scan, resulting in Detic features. In comparison, objects within $G_s$ derive their encodings from their names $l$, which are parsed via LLM during the input phase and are processed using the CLIP-text encoder. Thanks to the inherent alignment between Detic and CLIP-text features, object node distances between $G_s$ and $G_q$ can be computed seamlessly using Eq.\ref{eq:similarity}.

In the context of agent and region nodes, $G_s$ identifies them by the user-input names, $L_u$, whereas in $G_q$, these nodes are discerned by names $l$. For both, Sentence-BERT\cite{sentence-bert} serves as the encoding mechanism for linguistic features.

Delving into relationships, we distinguish spatial from abstract relationships. For $G_s$, spatial relationships are inferred from node positions, while in $G_q$, they're extracted from linguistic descriptions $l$ decoded from $L_q$ by the LLM. Given the absence of a standardized approach for spatial-language encoding, we innovated a spatial encoder, detailed in Appendix~\ref{appendix:sre}. Transitioning to abstract relationships, both $G_s$ and $G_q$ use language inputs — $l$ from user input, $L_u$ for the former, and text for the latter. GloVe effectively encodes this linguistic data across both domains.}


\textcolor{blue}{In discussing our design decisions, we highlight the intentional diversity in our feature encoding. Specifically, even for purely linguistic input, we harness the strengths of both GloVe and Sentence-BERT. Each encoder excels in unique areas; for instance, GloVe is adept at capturing subtle linguistic nuances, making it ideal for distinguishing abstract relationships like `like" and `dislike". In contrast, Sentence-BERT's lack of a fixed vocabulary allows it to more flexibly encode agent and region names.

This multi-encoder strategy isn't just about performance enhancement—it also offers design versatility. OVSG's modular architecture ensures that developers can seamlessly integrate new types and feature encoders in the future. It's worth noting that features from different embedding spaces are not compared directly, preserving the integrity and specificity of each encoder's output.}



\item \textbf{Grounding Accuracy} For each query, this metric computes the 3D IoU between the point cloud indices ($\mathbf{IoU_{3D-PCI}}$) of the system's predicted instance and the actual ground-truth instance.

[Whole Queries] ScanNet Grounding Accuracy(%)                                				
3D Point Cloud Index IoU > x	Method			
	OVIR-3D	OVSG-J	OVSG-S	OVSG-L
x = 0.15	57.58	32.79	65.57	83.77
x = 0.25	54.27	30.91	62.49	79.23
x = 0.50	43.86	24.83	51.22	63.88
x = 0.75	20.93	12.39	24.74	30.57

[Object-only Queries] ScanNet Grounding Accuracy(%)								
3D Point Cloud Index IoU > x	Method			
	OVIR-3D	OVSG-J	OVSG-S	OVSG-L
x = 0.15	59.94	24.77	63.97	81.88
x = 0.25	56.45	22.68	60.06	76.87
x = 0.50	45.13	17.22	47.79	60.35
x = 0.75	21.05	8.04	22.11	27.79

[Whole Queries] Dove-G Grounding Accuracy(%)                                				
3D Point Cloud Index IoU > x	Method			
	OVIR-3D	OVSG-J	OVSG-S	OVSG-L
x = 0.15	57.5	30.75	63.25	80.75
x = 0.25	55.25	30.75	61	78.5
x = 0.50	41.5	25.25	50.25	65.75
x = 0.75	16.25	12.5	25	32.25

[Object-only Queries] Dove-G Grounding Accuracy(%)                                				
3D Point Cloud Index IoU > x	Method			
	OVIR-3D	OVSG-J	OVSG-S	OVSG-L
x = 0.15	63.13	21.25	65.94	81.57
x = 0.25	61.57	21.25	64.38	80
x = 0.50	49.69	18.44	53.13	67.82
x = 0.75	18.13	5.63	20.32	28.75
[Whole Queries] ICL Grounding Accuracy(%)				
3D Point Cloud Index IoU > x	Method			
	OVIR-3D	OVSG-J	OVSG-S	OVSG-L
x = 0.15	52.65	51.26	72.99	93.88
x = 0.25	52.65	49.87	71.87	92.76
x = 0.50	45.97	44.29	61.84	78.56
x = 0.75	11.15	16.44	22.57	32.32

[Object-only Queries] ICL Grounding Accuracy(%)				
3D Point Cloud Index IoU > x	Method			
	OVIR-3D	OVSG-J	OVSG-S	OVSG-L
x = 0.15	56.85	33.16	65.79	89.48
x = 0.25	56.85	32.11	64.22	87.9
x = 0.50	48.95	22.64	51.58	68.95
x = 0.75	10	3.16	13.69	22.64


\begin{table}[htbp]
\centering
\scalebox{0.7}{
\begin{tabular}{>{\centering\arraybackslash}m{2.5cm}c>{\centering\arraybackslash}m{1.5cm}cccccccc}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Query Type} & \multirow{2}{*}{\# Queries} & \multicolumn{4}{c}{Avg. Top1 $\mathbf{IoU_{BB}}$ per Query} & \multicolumn{4}{c}{Avg. Top3 $\mathbf{IoU_{BB}}$ per Query} \\
\cmidrule(lr){4-7} \cmidrule(lr){8-11}
& & & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L & OVIR-3D & OVSG-J & OVSG-S & \cellcolor{PaleBlue}OVSG-L \\ 
\midrule
\multirow{2}{*}{ScanNet} & Object-only & 18,863 & 0.38 & 0.15 & 0.4 & \cellcolor{PaleBlue}\textbf{0.51} & 0.52 & 0.4 & 0.52 & \cellcolor{PaleBlue}\textbf{0.55} \\
& Whole & 20,173 & 0.37 & 0.22 & 0.44 & \cellcolor{PaleBlue}\textbf{0.55} & 0.53 & 0.45 & 0.55 & \cellcolor{PaleBlue}\textbf{0.57} \\
\addlinespace[0.5em]
\multirow{2}{*} {DOVE-G} & Object-only & 320 & 0.37 & 0.14 & 0.39 & \cellcolor{PaleBlue}\textbf{0.49} & 0.57 & 0.36 & \cellcolor{PaleBlue}\textbf{0.56} & \cellcolor{PaleBlue}\textbf{0.56} \\
& Whole & 400 & 0.35 & 0.2 & 0.41 & \cellcolor{PaleBlue}\textbf{0.51} & 0.55 & 0.41 & 0.55 & \cellcolor{PaleBlue}\textbf{0.56} \\
\addlinespace[0.5em]
\multirow{2}{*} {ICL-NUIM} & Object-only & 190 & 0.32 & 0.18 & 0.37 & \cellcolor{PaleBlue}\textbf{0.5} & 0.55 & 0.49 & 0.55 & \cellcolor{PaleBlue}\textbf{0.56} \\
& Whole & 359 & 0.33 & 0.34 & 0.47 & \cellcolor{PaleBlue}\textbf{0.61} & 0.62 & 0.56 & \cellcolor{PaleBlue}\textbf{0.64} & \cellcolor{PaleBlue}\textbf{0.64} \\
\bottomrule
\end{tabular}
}
\caption{\color{blue} 3D Bounding Box IoU averaged over all queries in ScanNet, DOVE-G, and ICL-NUIM datasets}
\label{tab:add2}
\end{table}
